Global existence for vector valued fractional reaction-diffusion equations

In this paper, we study the initial value problem for infinite dimensional fractional non-autonomous reaction-diffusion equations. Applying general time-splitting methods, we prove the existence of solutions globally defined in time using convex sets as invariant regions. We expose examples, where biological and pattern formation systems, under suitable assumptions, achieve global existence. We also analyze the asymptotic behavior of solutions.

==> def.tex <==

%\renewcommand{\thechapter}{\Roman{chapter}}


%%%%% EQUATIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\numberwithin{equation}{section}

%%%%% THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newtheorem{corollary}{Corolario}[section]
%\newtheorem{lemma}{Lema}[section]
%\newtheorem{proposition}{Proposición}[section]
%\newtheorem{theorem}{Teorema}[section]

%%%%% demS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\renewenvironment{proof}[1][Demostraci\'on]{\noindent \textbf{#1.} }{\rule{0.5em}{0.5em}}

%%%%% DEFINITIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{definition}

\newtheorem{conjeture}{Conjetura}[section]
%\newtheorem{definition}{Definición}[section]
%\newtheorem{example}{Ejemplo}[section]
%\newtheorem{remark}{Observación}[section]
\newtheorem{exercise}{Ejercicio}[section]
{\swapnumbers\newtheorem{exercisestar}[exercise]{(*)}}
\newenvironment{sol}[1][\textbf{Solución:}]
{\noindent #1 \noindent \small}


%%%%% NUMERICAL SETS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}

%%%%% FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\abs}[1]{\ensuremath{\left\vert #1\right\vert}}
\newcommand{\ket}[1]{\ensuremath{\left| #1 \right\rangle}}
\newcommand{\set}[1]{\ensuremath{\left\{ #1\right\}}}
\newcommand{\norm}[1]{\ensuremath{\left\|#1\right\|}}
\newcommand{\pa}[1]{\ensuremath{\left(#1\right)}}
\newcommand{\pro}[2]{\ensuremath{\langle #1|#2 \rangle}}
\newcommand{\proo}[3]{\ensuremath{\langle #1|#2|#3 \rangle}}
\newcommand{\Rn}[1][n]{\ensuremath{\mathbb{R}^{#1}}}
\newcommand{\Cn}[1][n]{\ensuremath{\mathbb{C}^{#1}}}
\newcommand{\sgn}[1]{\ensuremath{\mathrm{sgn}\pa{#1}}}
\newcommand{\ran}[1]{\mathrm{Ran}\pa{#1}}
\newcommand{\tr}[1]{\mathop{\mathrm{tr}}\pa{#1}}

\newcommand{\hil}[1][X]{\ensuremath{\mathrm{#1}}}
\newcommand{\ham}[1][H]{\ensuremath{\mathcal{#1}}}
\newcommand{\kam}[1][H]{\ensuremath{\mathcal{#1}}}

\renewcommand{\Re}[1]{\ensuremath{\mathrm{Re}\left( #1\right)}}
\renewcommand{\Im}[1]{\mathrm{Im}\left( #1\right)}
\renewcommand{\exp}[1]{\mathrm{exp}\left( #1\right)}
%\renewcommand{\exp}[1]{e^{#1}}
\renewcommand{\cos}[1]{\mathrm{cos}\left( #1\right)}
\renewcommand{\sin}[1]{\mathrm{sen}\left( #1\right)}
%\newcommand{\id}{\mathds{1}}


\newcommand{\num}[3]{\ensuremath{#1\times 10^{#2}\,\mathrm{#3}}}
\newcommand{\al}{&\,}
